A Study on the Impact of Environmental Liability Insurance on Industrial Carbon Emissions

In order to explore whether environmental liability insurance has an important impact on industrial emission reduction, this paper selects provincial (city) level panel data from 2010 to 2020 and constructs a two-way fixed effect model to analyze the impact of environmental liability insurance on carbon emissions from both direct and indirect levels. The empirical analysis results show that: at the direct level, the development of environmental liability insurance has the effect of reducing industrial carbon emissions, and its effect is heterogeneous. At the indirect level, the role of environmental liability insurance is weaker in areas with developed financial industry and underdeveloped financial industry. Further heterogeneity analysis shows that in the industrial developed areas, the effect of environmental liability insurance on carbon emissions is more obvious. Based on this, countermeasures and suggestions are put forward from the aspects of expanding the coverage of environmental liability insurance, innovating the development of environmental liability insurance and improving the level of industrialization.

==> algorithms/gla_scan_1.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
        
%
%

%
%
%
%
        
%
%
%
%
%
%
%
%
%
%
%
%


%
%
%
%
%
%
%
%
%
%
%

    
%

%

%
%

%

%

%
%
%
    
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

   
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
  
%
%




%
%
%
%
%
%
%
%
%
%
%

%
     

%

%

%
%

%

%

        
%
%
%

       
%
%
%


%
%
         
%
%

%
%
%

%

%
%
%

%

        
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
  
%
%


\begin{algorithm}[b!]
\footnotesize
\caption{Forward pass for gated linear attention (w. materialization)}
\label{algo:gla-chunk-scan-1-fwd}
\begin{algorithmic}
    \Require $\rmQ, \rmK, \in \R^{L \times d_k}, \rmV  \in \R^{L \times d_v}$, $\rmG =[\balpha_1 \dots \balpha_L] \in \R^{L \times d_k}$, chunk size $C$
    \State Divide $\rmQ, \rmK, \rmG$ into $N = \frac{L}{C}$ blocks $\{ \rmQ_{[1]} \dots \rmQ_{[N]} \} $, $\{ \rmK_{[1]} \dots \rmK_{[N]} \}$, $\{ \rmG_{[1]} \dots \rmG_{[N]} \} $ of size $C \times d_k$ each.
    \State Divide $\rmV$ into $N$ blocks $\{ \rmV_{[1]} \dots \rmV_{[N]} \}$ of size $C \times d_v$ each.
     \State{Initialize $\rmS = \bm{0} \in \mathbb R^{d_k\times d_v} $ on SRAM}
    \For{$n \gets 1, N$}
      \State{Write $\mathbf S$ to HBM as $\rmS_{[n]}$.} 
        \State Load $\rmK_{[n]}, \rmG_{[n]} \in \R^{C \times d_k}$ from HBM to SRAM. 
        \State Load $\rmV_{[n]} \in \R^{C \times d_v}$ from HBM to SRAM.
        \State On chip, compute $\bgamma_{[n]} \in \R^{d_k}, \bGamma_{[n]} \in \R^{C \times d_k}$ and $\tilde \rmK_{[n]} = \rmK_{[n]} \odot \bGamma_{[n]}$. %
        \State{On chip, compute $\rmS = \left(\bgamma_{[n]}^\intercal\mathbf{1}\right) \odot \mathbf{S} + \tilde \rmK_{[n]}^{\top}  \rmV_{[n]}$.}  
        %
    \EndFor
   \ParFor{$n \gets 1, N$}
        \State Load $\rmQ_{[n]}, \rmK_{[n]}, \rmG_{[n]} \in \R^{C \times d_k}$ from HBM to SRAM.
        \State Load $\rmV_{[n]}  \in \R^{C \times d_v}$ from HBM to SRAM.
        \State Load $\rmS_{[n]} \in \R^{d_k \times d_v}$ from HBM to SRAM.
        \State On chip, construct causal mask $\rmM\in \R^{C \times C}$ %
        \State On chip, compute $\bLambda_{[n]}, \bGamma_{[n]} \in \R^{C \times d_k}$
        \State On chip, compute $\tilde \rmQ_{[n]} = \rmQ_{[n]} \odot \bLambda_{[n]}$, $\tilde \rmK_{[n]} = \rmK_{[n]} \odot \bGamma_{[n]}$, $\bar \rmK_{[n]} = \rmK_{[n]} / \bLambda_{[n]}$
        \State On chip, compute $\rmO_{[n]}^{\text{inter}} = \tilde \rmQ_{[n]} \rmS_{[n]} \in \R^{C \times d_v}$
        \State On chip, compute $\rmP = (\tilde \rmQ_{[n]} \bar \rmK^\intercal_{[n]})\odot \rmM  \in \R^{C \times C} $
        \State On chip, compute $\rmO^{\text{intra}} = \rmP \rmV_{[n]} $ 
        \State On chip, compute $ \rmO_{[n]} = \rmO^{\text{inter}} + \rmO^{\text{intra}} $
        \State Store $\rmO_{[n]}$ to HBM.
   \EndParFor
  \State \Return $\rmO = \{ \rmO_{[1]} \dots \rmO_{[N]} \}$, $\rmS=\{ \rmS_{[1]} \dots \rmS_{[N]} \}$.
\end{algorithmic}
\end{algorithm}
\begin{algorithm}[tbh!]
\footnotesize
\caption{Backward pass for gated linear attention (w. materialization)}
\label{algo:gla-chunk-scan-1-bwd}
\begin{algorithmic}
    \Require $\rmQ, \rmK, \rmG \in \R^{L \times d_k}$, $\rmV, \rmO, \rmdO \in \R^{L \times d_v}$, chunk size $C$
     \State{Initialize $\rmdS = \bm{0} \in \mathbb R^{d_k\times d_v} $ on SRAM}
    \For{$n \gets N, 1$} %
        \State Store $\rmdS$ in HBM as $\rmdS_{[n]}$
        \State{Load $\rmG_{[n]}  \in \R^{C \times d_k}$ from HBM to SRAM.}
        \State{Load $\rmQ_{[n]}  \in \R^{C \times d_k}$ from HBM to SRAM.}
        \State{Load $\rmdO_{[n]}  \in \R^{C \times d_v}$ from HBM to SRAM.}
        \State On chip, compute $\bgamma_{[n]}$, $\bGamma_{[n]}$ and $\tilde \rmQ{[n]} =  \rmQ_{[n]} \odot \bGamma{[n]}$
        \State On chip, compute $\rmdS = \left(\bgamma_{[n]}^\intercal\mathbf{1}\right) \odot \rmdS + \tilde \rmQ_{[n]}^\intercal \rmdO_{[n]}$
      \EndFor
      \ParFor{$n \gets 1, N$}
        \State{Load $\rmQ_{[n]}, \rmK_{[n]}, \rmG_{[n]} \in \R^{C \times d_k}$ from HBM to  SRAM.}
        \State Load $\rmS_{[n]} \in \R^{d_k \times d_v}$ from HBM to  SRAM.
        \State Load $\rmV_{[n]}, \rmO_{[n]}, \rmdO_{[n]} \in \R^{C \times d_v}$ from HBM to  SRAM.
        \State Load $\rmdS_{[n]} \in \R^{d_k \times d_v}$ from HBM to SRAM.
        \State On chip, construct causal mask $\rmM\in \R^{B\times B}$ %
        \State On chip, compute $\bLambda_{[n]}, \bGamma_{[n]} \in \R^{C \times d_k}$
        \State On chip, compute $\tilde \rmQ_{[n]} = \rmQ_{[n]} \odot \bLambda_{[n]}$, $\tilde \rmK_{[n]} = \rmK_{[n]} \odot \bGamma_{[n]}$, $\bar \rmK_{[n]} = \rmK_{[n]} / \bLambda_{[n]}$.
        \State On chip, compute $\rmP = (\tilde \rmQ_{[n]} \tilde \rmK^\intercal_{[n]})\odot \rmM  \in \R^{C \times C} $
        \State On chip, compute $\rmdP =( \rmdO_{[n]} \rmV_{[n]}^\intercal) \odot \rmM $
        \State On chip, compute $ \rmdbK_{[n]} = \tilde \rmQ_{[n]} \rmdP^\intercal$
        \State On chip, compute $ \rmdtK_{[n]} = \rmV_{[n]} \rmdS_{[n]}  ^\intercal$
        \State On chip, compute $\rmdK_{[n]} =  \rmdtK_{[n]} \odot \bGamma_{[n]}  + \rmdbK_{[n]} / \bLambda_{[n]} $
        \State{On chip, compute $\rmdtQ_{[n]} = \rmdP \, \bar \rmK_{[n]} + \rmdO_{[n]} \rmS_{[n]}^\intercal $}
        \State On chip, compute $\rmdQ_{[n]} =  \rmdtQ_{[n]} \odot \bLambda_{[n]} $
        \State On chip, compute $\rmdV_{[n]} = \rmP^\intercal \, \rmdO_{[n]} + \tilde \rmK_{[n]} \rmdS_{[n]} $
        \State Store $\rmdK_{[n]}, \rmdV_{[n]}$ in HBM.
      \EndParFor
  \State Let $\rmdQ = \{ \rmdQ_{[1]} \dots \rmdQ_{[N]} \}$, $\rmdK=\{ \rmdK_{[1]} \dots \rmdK_{[N]} \}$, $\rmdV=\{ \rmdV_{[1]} \dots \rmdV_{[N]} \}$.
  \State Compute $\rmdA = \rmQ \odot \rmdQ - \rmK \odot \rmdK $, $\rmdG = \revcum(\rmdA) $
  \State \Return $\rmdQ, \rmdK, \rmdV, \rmdG$
\end{algorithmic}
\end{algorithm}



==> algorithms/gla_scan_2.tex <==
\begin{algorithm}[b!]
\small
\caption{Forward pass for gated linear attention (w/o. materialization)}
\label{algo:gla-chunk-scan-2-fwd}
\begin{algorithmic}
    \Require $\rmQ, \rmK, \in \R^{L \times d_k}, \rmV  \in \R^{L \times d_v}$, $\rmG =[\balpha_1 \dots \balpha_L] \in \R^{L \times d_k}$, chunk size $C$
    \State Divide $\rmQ, \rmK, \rmG$ into $N = \frac{L}{B}$ blocks $\{ \rmQ_{[1]} \dots \rmQ_{[N]} \} $, $\{ \rmK_{[1]} \dots \rmK_{[N]} \}$, $\{ \rmG_{[1]} \dots \rmG_{[N]} \} $ of size $C \times d_k$ each.
    \State Divide $\rmV$ into $N$ blocks $\{ \rmV_{[1]} \dots \rmV_{[N]} \}$ of size $C \times d_v$ each.
     \State{Initialize $\rmS = \bm{0} \in \mathbb R^{d_k\times d_v} $ on SRAM}
    \For{$n \gets 1, N$}
      \State{Write $\mathbf S$ to HBM as $\rmS_{[n]}$.} 
        \State Load $\rmQ_{[n]}, \rmK_{[n]}, \rmG_{[n]} \in \R^{C \times d_k}$ from HBM to SRAM.
        \State Load $\rmV_{[n]}  \in \R^{C \times d_v}$ from HBM to SRAM.
        \State On chip, compute $\bgamma_{[n]} \in \R^{d_k}, \bGamma_{[n]} \in \R^{C \times d_k}$ and $\tilde \rmK_{[n]} = \rmK_{[n]} \odot \bGamma_{[n]}$. %
        \State On chip, construct causal mask $\rmM\in \R^{C\times C}$ %
        \State On chip, compute $\bLambda_{[n]}, \bGamma_{[n]} \in \R^{C \times d_k}$
        \State On chip, compute $\tilde \rmQ_{[n]} = \rmQ_{[n]} \odot \bLambda_{[n]}$, $\tilde \rmK_{[n]} = \rmK_{[n]} \odot \bGamma_{[n]}$, $\bar \rmK_{[n]} = \rmK_{[n]} / \bLambda_{[n]}$.
        \State On chip, compute $\rmO_{[n]}^{\text{inter}} = \tilde \rmQ_{[n]} \rmS_{[n]} \in \R^{C \times d_v}$
        \State On chip, compute $\rmP = (\tilde \rmQ_{[n]} \bar \rmK^\intercal_{[n]})\odot \rmM  \in \R^{C \times C} $
        \State On chip, compute $\rmO^{\text{intra}} = \rmP \rmV_{[n]} $
        \State On chip, compute $ \rmO_{[n]} = \rmO^{\text{inter}} + \rmO^{\text{intra}} $
        \State Store $\rmO_{[n]}$ to HBM.
        \State{On chip, compute $\rmS = \left(\bgamma_{[n]}^\intercal \mathbf{1}\right) \odot \mathbf{S} + \tilde \rmK_{[n]}^{\top}  \rmV_{[n]}$.}  
   \EndFor
  \State \Return $\rmO = \{ \rmO_{[1]} \dots \rmO_{[N]} \}$.
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[tbh!]
\small
\caption{Backward pass for gated linear attention (w/o. materialization)}
\label{algo:gla-chunk-scan-2-bwd}
\begin{algorithmic}
    \Require $\rmQ, \rmK, \rmG \in \R^{L \times d_k}$, $\rmV, \rmO, \rmdO \in \R^{L \times d_v}$, chunk size $C$
    \State{Initialize $\rmS = \bm{0} \in \R^{d_k\times d_v} $ on SRAM}
    \For{$n \gets 1, N$} %
        %
        \State{Load $\rmG_{[n]}  \in \R^{C \times d_k}$ from HBM to SRAM.}
        \State{Load $\rmQ_{[n]}  \in \R^{C \times d_k}$ from HBM to SRAM.}
        \State{Load $\rmdO_{[n]}  \in \R^{C \times d_v}$ from HBM to SRAM.}
        \State On chip, compute $\bgamma_{[n]} \in \R^{d_k}, \bGamma_{[n]} \in \R^{C \times d_k}$ and $\tilde \rmK_{[n]} = \rmK_{[n]} \odot \bGamma_{[n]}$.
        \State On chip, compute $\rmdP = \rmdO_{[n]} \rmV_{[n]}^\intercal $
        \State{On chip, compute $\rmdtQ_{[n]} = \rmdP \, \tilde \rmK_{[n]} + \rmdO_{[n]} \rmS^\intercal $}
        \State On chip, compute $\rmdQ= \rmdtQ_{[n]} \odot \bGamma{[n]} $
        \State Store $\rmdQ_{[n]}$ to HBM.
        \State{On chip, compute $\rmS = \left(\bgamma_{[n]}^\intercal\mathbf{1}\right) \odot \mathbf{S} + \tilde \rmK_{[n]}^{\top}  \rmV_{[n]}$.}  
      \EndFor
    \State{Initialize $\rmdS = \bm{0} \in \mathbb R^{d_k\times d_v} $ on SRAM}
      \For{$n \gets N, 1$}
        \State{Load $\rmQ_{[n]}, \rmK_{[n]}, \rmG_{[n]} \in \R^{C \times d_k}$ from HBM to  SRAM.}
        %
        \State Load $\rmV_{[n]}, \rmO_{[n]}, \rmdO_{[n]} \in \R^{C \times d_v}$ from HBM to  SRAM.
        \State On chip, construct causal mask $\rmM\in \R^{C\times C}$ %
        \State On chip, compute $\bLambda_{[n]}, \bGamma_{[n]} \in \R^{C \times d_k}$
        \State On chip, compute $\tilde \rmQ_{[n]} = \rmQ_{[n]} \odot \bLambda_{[n]}$, $\tilde \rmK_{[n]} = \rmK_{[n]} \odot \bGamma_{[n]}$.
        \State On chip, compute $\rmP = (\tilde \rmQ_{[n]} \tilde \rmK^\intercal_{[n]})\odot \rmM  \in \R^{C \times C} $
        \State On chip, compute $\rmdP = (\rmdO_{[n]} \rmV_{[n]}^\intercal) \odot \rmM $
                \State On chip, compute $ \rmdbK_{[n]} = \tilde \rmQ_{[n]} \rmdP^\intercal$
        \State On chip, compute $ \rmdtK_{[n]} = \rmV_{[n]} \rmdS_{[n]}  ^\intercal$
        \State On chip, compute $\rmdK_{[n]} =  \rmdtK_{[n]} \odot \bGamma_{[n]}  + \rmdbK_{[n]} / \bLambda_{[n]} $
        \State On chip, compute $\rmdV_{[n]} = \rmP^\intercal \, \rmdO_{[n]} + \tilde \rmK_{[n]} \rmdS $
        \State Store $\rmdQ_{[n]}, \rmdK_{[n]}, \rmdV_{[n]}$ in HBM.
        \State On chip, compute $\rmdS = \left(\bgamma_{[n]}^\intercal \mathbf{1} \right) \odot \rmdS + \tilde \rmQ_{[n]}^\intercal \rmdO_{[n]}$
      \EndFor
  \State Let $\rmdQ = \{ \rmdQ_{[1]} \dots \rmdQ_{[N]} \}$, $\rmdK=\{ \rmdK_{[1]} \dots \rmdK_{[N]} \}$, $\rmdV=\{ \rmdV_{[1]} \dots \rmdV_{[N]} \}$.
  \State Compute $\rmdA = \rmQ \odot \rmdQ - \rmK \odot \rmdK $, $\rmdG = \revcum(\rmdA) $
  \State \Return $\rmdQ, \rmdK, \rmdV, \rmdG$
\end{algorithmic}
\end{algorithm}

==> algorithms/la-chunk-bwd.tex <==

\begin{algorithm}[hb]
\scriptsize
\caption{\textsc{FlashLinearAttention}: Backward Pass}
\label{algo:la-chunk-bwd}
\begin{algorithmic}
    \Require $\rmQ, \rmK, \rmV, \rmO, \rmdO \in \R^{L \times d}$, chunk size $C \in [L]$,  \texttt{materialize} $\in$ \{\texttt{True,False}\}, $\rmS \in \R^{\frac{L}{C} \times d \times d}$ \Comment{$\rmS$ is available when \texttt{materialize} is True}
 \State{Initialize $\rmdS = \bm{0} \in \mathbb R^{d\times d} $ on SRAM}
         \State On chip, construct causal mask $\rmM\in \R^{C\times C}$ %
             %
%
%
%
%
%
%
%
%
%
%
\If{\texttt{materialize}} \Comment{the materialization version}
\color{black}
    \For{$n \gets N, 1$}   \Comment{in reverse order}
        \State Store $\rmdS$ in HBM as $\rmdS_{[n]}$
    \color{black}
        \State{Load $\rmQ_{[n]}, \rmdO_{[n]}  \in \R^{C \times d}$ from HBM to SRAM.}
        \State On chip, compute $\rmdS = \rmdS + \rmQ_{[n]}^\intercal \rmdO_{[n]}$
        \color{orange}
       %
       %
       %
       %
       %
       %
       %
            \color{black}
      \EndFor
      %
    %
      \ParFor{$n \gets 1, N$}  
        \State{Load $\rmQ_{[n]}, \rmK_{[n]},\rmV_{[n]}, \rmdO_{[n]} \in \R^{C \times d}$ from HBM to  SRAM.}
        \State{Load $ \rmS_{[n]}$, $\rmdS_{[n]} \in \R^{d \times d}$ from HBM to SRAM.}
        %
        %
        %
        %
        %
        %
        %
        %
        %

   \State On chip:  $\mathbf{dQ} = \mathbf{dO}_{[n]} \rmS_{[n]}^{\top}  + (\mathbf{dO}_{[n]} \rmV_{[n]}^{\top} \odot \mathbf{M}) \mathbf{K}_{[n]}$.
   \State On chip:   $\mathbf{dK} =  \mathbf{V}_{[n]} \mathbf{dS}_{[n]}^{\top} +  (\mathbf{V}_{[n]}\mathbf{dO}_{[n]}^{\top} \odot \mathbf{M}^{\top}) \mathbf{Q}_{[n]}$
   \State On chip: $\mathbf{dV} =  \mathbf{K}_{[n]} \mathbf{dS}_{[n]} + (\rmQ_{[n]}\rmK_{[n]}^{\top} \odot \mathbf{M})^{\top} \mathbf{dO}_{[n]}$
    \State Write $ \mathbf {dQ}, \mathbf{dK}, \mathbf{dV}$ to HBM as $\mathbf{dQ}_{[n]}, \mathbf{dK}_{[n]}, \mathbf{dV}_{[n]}$
      \EndParFor
      %
      \color{black}
\Else  \Comment{the non-materialization version}
\State Initial $\rmS = \bm{0} \in \mathbb R^{d\times d} $ on SRAM
\For{$n \gets 1, N$}    \Comment{hidden state recomputation}
\State Load $\rmK_{[n]}, \rmV_{[n]}, \rmdO_{[n]}   \in \R^{C \times d}$ from HBM to SRAM.
%
\State On chip: $\rmdQ = \mathbf{dO}_{[n]} \rmS^{\top}  + (\mathbf{dO}_{[n]} \rmV_{[n]}^{\top} \odot \mathbf{M}) \mathbf{K}_{[n]}$ 
\State On chip: $\rmS = \rmS + \rmK_{[n]}^{\top}\rmV_{[n]}$
\EndFor
\color{black}
    \For{$n \gets N, 1$}   \Comment{in reverse order}
    \color{black}
        \State{Load $\rmQ_{[n]},\rmK_{[n]}, \rmV_{[n]}, \rmdO_{[n]}  \in \R^{C \times d}$ from HBM to SRAM.}
        \State On chip, compute $\rmdS = \rmdS + \rmQ_{[n]}^\intercal \rmdO_{[n]}$
        %
       \State On chip:  $\mathbf{dQ} = \mathbf{dO}_{[n]} \rmS_{[n]}^{\top}  + (\mathbf{dO}_{[n]} \rmV_{[n]}^{\top} \odot \mathbf{M}) \mathbf{K}_{[n]}$.
       \State On chip:   $\mathbf{dK} = \mathbf{V}_{[n]}\mathbf{dS}_{[n]}^{\top}  +  (\mathbf{V}_{[n]}\mathbf{dO}_{[n]}^{\top} \odot \mathbf{M}^{\top}) \mathbf{Q}_{[n]}$
       \State On chip: $\mathbf{dV} =  \mathbf{K}_{[n]} \mathbf{dS}_{[n]} + (\rmQ_{[n]}\rmK_{[n]}^{\top} \odot \mathbf{M})^{\top} \mathbf{dO}_{[n]}$
           \State Write $ \mathbf {dQ}, \mathbf{dK}, \mathbf{dV}$ to HBM as $\mathbf{dQ}_{[n]}, \mathbf{dK}_{[n]}, \mathbf{dV}_{[n]}$
            \color{black}
      \EndFor
\EndIf 
  \State \Return $\rmdQ = \{ \rmdQ_{[1]} \dots \rmdQ_{[N]} \}$, $\rmdK=\{ \rmdK_{[1]} \dots \rmdK_{[N]} \}$, $\rmdV=\{ \rmdV_{[1]} \dots \rmdV_{[N]} \}$.
\end{algorithmic}
\end{algorithm}


==> algorithms/la-chunk-fwd.tex <==
\begin{algorithm}[t!]
\vspace{-0.5mm}
\scriptsize
\caption{\textsc{FlashLinearAttention}: Forward Pass}
\label{algo:la-chunk-fwd}
\begin{algorithmic}
    \Require $\rmQ, \rmK, \rmV \in \R^{L \times d}, \rmV  \in \R^{L \times d}$, chunk size $C \in [L]$, \texttt{materialize} $\in$ \{\texttt{True,False}\} 
    \State Divide $\rmQ, \rmK, \rmV$ into $N = \frac{L}{C}$ blocks $\{ \rmQ_{[1]} \dots \rmQ_{[N]} \} $, $\{ \rmK_{[1]} \dots \rmK_{[N]} \}$ of size $C \times d$ each.
     \State{Initialize $\rmS = \bm{0} \in \mathbb R^{d\times d} $ on SRAM}
    \State{On chip, construct causal mask $\rmM\in \R^{C\times C}$}
    \If{\texttt{materialize}} \Comment{the materialization version}
    \For{$n \gets 1, N$}
    %
    %
      \State{Store $\rmS$ to HBM as 
      $\rmS_{[n]}$.}
      %
      %
      %
        \State{Load $\rmK_{[n]}, \rmV_{[n]} \in \mathbb{R}^{C \times d}$ from HBM to SRAM}
        \State{On chip, compute $\mathbf{S} = \mathbf{S} + \rmK_{[n]}^{\top}  \rmV_{[n]}$.}
        %
        %
        %
        %
        %
        %
        \color{black}
    \EndFor
    %
    %
    \ParFor{$n \gets 1, N$}
    %
        \State Load $\rmQ_{[n]}, \rmK_{[n]}, \rmV_{[n]}, \rmS_{[n]}$ from HBM to SRAM.
        \State On chip, compute $\rmO^{\prime} = \rmQ_{[n]} \rmS_{[n]} + (\rmQ_{[n]} \rmK^\intercal_{[n]} \odot \rmM)\rmV_{[n]}$  
        \State Store $\rmO^{\prime}$ to HBM as $\rmO_{[n]}$.
    \EndParFor
  \State \Return $\rmO = \{ \rmO_{[1]} \dots \rmO_{[N]} \}$, $\rmS=\{ \rmS_{[1]} \dots \rmS_{[N]} \}$.
        \Else \Comment{the non-materialization version}
         \For{$n \gets 1, N$}
      \color{black}
        \State{Load $\rmQ_{[n]}, \rmK_{[n]}, \rmV_{[n]} \in \mathbb{R}^{C \times d}$ from HBM to SRAM}
        %
        \State{On chip, compute $\rmO' = \rmQ_{[n]}\rmS + (\rmQ_{[n]}\rmK_{[n]}^{\top}\odot\rmM)\rmV_{[n]}$}
        \State{On chip, compute $\mathbf{S} = \mathbf{S} + \rmK_{[n]}^{\top}  \rmV_{[n]}$.}
        \State{Store $\rmO'$ to HBM as $\rmO_{[n]}$ }
        \color{black}
    \EndFor
   \State  \Return $\rmO = \{ \rmO_{[1]} \dots \rmO_{[N]} \}$   
\EndIf 
%
  %
%
%
%
\vspace{-0.5mm}
\end{algorithmic}
\end{algorithm}


==> sections/ack.tex <==
\section*{Impact Statement}
%
%

This paper aims to improve the training efficiency of a new model family of (gated) linear attention models. The efficiency advantage of such models might help democratize access of language models. On the other hand, whether such new architectures would affect known issues such as biased and harmful outputs of language models remains an unexplored research question.

\section*{Acknowledgments}

This work was supported by MIT-IBM Watson AI Lab. We thank Yutao Sun, Zhen Qin, Li Dong, Xinyu Yang, Jiacheng You, Huanqi Cao, Yu Zhang, and Shida Wang for their insightful discussions. We also thank Yu Zhang, Fares Obeid, Daniel Goldstein, and Liliang Ren for their proofreading. Special thanks to Yu Zhang for contributing to the \textsc{FlashLinearAttention} library.


==> sections/related.tex <==
\vspace{-2mm}
\section{Related Work}
\label{sec:related}
\vspace{-2mm}
We briefly discuss related work here and give an extended discussion of the related work in Appendix~\ref{appdx:extended_rw}.
%

Traditional RNNs are difficult to scale  due to the nonlinear dependencies between the  hidden states and expensive matmul-based sequential hidden state updates. Linear RNNs/State-Space Models (SSMs)/Transformers eliminate nonlinear dependencies, making training parallelizable along the temporal dimension \citep{parallel-martin, s4, s5}. Such models have been the focus of much recent work as a competitive sub-quadratic alternative to the Transformer architecture \citep{rwkv, Gu2023MambaLS,HGRN,qin2023scaling,sun2023retentive,pretrain_wo_attn}.



\input{figures/tps}



Data-dependent decay rates have always been regarded important for  RNNs  \citep{DBLP:journals/neco/GersSC00,unreasonable-forget-gate}. Typical forget gate values depend on both the previous hidden state and the current input. However \citet{parallel-martin} suggest that forget gate values should depend solely on the current inputs to enable parallel training. This simple strategy has been shown to be effective in moderate-scale experiments conducted by HGRN \citep{qin2023scaling}.  RWKV-v6 \citep{peng2024eagle} and Mamba \citep{Gu2023MambaLS} also use data-dependent decay rates that are reminiscent of forget gates. In the context of linear Transformers, \citet{peng2021random} employ a coarse-grained position-wise forget gate, while \citet{mao-2022-fine} and \citet{gatedloop} use a more fine-grained forget gate. 
%

RNNs rely on fixed-dimensional hidden states to encode their entire history. The hidden state dimension  serves as a proxy for memory capacity and thus significantly influences their expressive power. 
Linear Transformers expand the hidden dimension of RNNs via the outer-product parameterization, as discussed \S\ref{subsec:background-lin}. Linear SSMs on the other hand expand their hidden dimension via a single-input-single-output (SISO) strategy. 
Without data-dependent SSM parameters, this can be done efficiently during training via the Fast Fourier Transform (FFT). However, with data-dependent SSM parameters, FFT-based training is not possible, and thus \citet{Gu2023MambaLS} implements a custom CUDA kernel to train a selective state-space model using the parallel scan algorithm \citep{s5}. To fit all the hidden states into SRAM, they can only afford an expansion rate up to 16. In contrast our hardware-aware training algorithm provides an alternative, efficient approach for expanding the hidden dimension to a wider range, which we have shown useful in recall-intensive tasks.


\vspace{-2mm}
%
%







==> sections/supp_alg.tex <==
\section{Extended Related Work }
\label{appdx:extended_rw}
\vspace{2mm}




\subsection{Linear Attention}

\paragraph{Feature map $\phi$.} Linear attention mechanisms~\citep{katharopoulos2020transformers} replace $\exp(\vq_t \vk_i^\intercal)$ with a kernel $k(\vx, \vy)$ having an associated feature map $\phi$ (i.e., $k(\vx, \vy) = \langle\phi(\vx), \phi(\vy)\rangle$) where $\phi \in \R^{d_{\text{key}}}\rightarrow \R^{d_{\text{dot}}}$.
$\phi$ often consists of two parts: $\phi = \phi_0 \circ \phi_1$. $\phi_1$ could be a linear map made up by random samples \cite{peng2021random, performer}, learnable MLPs \cite{kasai-etal-2021-finetuning, Hedgehog, polysketch} or simply an identity map \cite{mao-2022-fine}. $\phi_2$ is often an element-wise (activation) function that makes the resulting $\phi$ a positive feature map, such as $1+\operatorname{elu}$ \cite{katharopoulos2020transformers}, $\operatorname{ReLU}$ \cite{kasai-etal-2021-finetuning}, $\exp(\cdot)$ \cite{Hedgehog, performer}. Some work \cite{qin2023scaling, sun2023retentive, mao-2022-fine} suggests that a positive feature map might not be necessary.

Our work follows \citet{sun2023retentive} and \citet{mao-2022-fine} by using an identity map $\phi=\mathbf{I}$.  Recent work suggests that non-identity feature maps such as scaled element-wise exponential map  \cite{log-normal, Hedgehog}
and higher-order polynomial map \cite{Arora2024SimpleLA,polysketch} work well empirically. We leave the exploration of integrating other types of feature map into GLA to future work.


\paragraph{Attention spikiness.} Linear attention suffers from the ``attention dilution'' issue \citep{qin2022devil}, where the attention distribution is too uniform (i.e., high entropy) to concentrate on relevant tokens. \citet{qin2022devil} propose adding local attention layers to focus more on adjacent tokens, a method adopted in \citep{VQ-Transformer, log-normal, orthogonal_memory} and proven crucial for performance. 
Recent work finds that a scaled element-wise exponential map---i.e., $\phi(\mathbf{x})= \mathbf{\exp}(t\cdot \mathbf{x})$ with $t \ge 2$---helps to concentrate attention \cite{log-normal, Hedgehog}. \citet{Hedgehog} also find that higher-order polynomial kernels induce low-entropy and spiky attention distribution, partially explaining the empirical success of Based Linear Attention \cite{Arora2024SimpleLA} and PolySketchFormer \cite{polysketch}.



\paragraph{Memory capacity.} 
 Linear attention has bounded memory size \cite{peng-etal-2022-abc} while softmax attention enjoys unbounded memory\cite{Oren2024TransformersAM}. We believe that increasing the memory size efficiently and utilizing memory effectively are the keys to bridging the performance gap between linear attention and softmax attention. To increase memory size, it is shown that  directly increasing $d_{\operatorname{key}}$ is effective \citep{sun2023retentive, mao-2022-fine, zhang-cai-2022-linearizing}; however, the total parameters are hard to control with the increase of $d_{\operatorname{key}}$.
 Parameter-efficient methods often keep $d_{\text{key}}$ intact and increase $d_{\text{dot}}$ instead. Higher order polynomial kernels with order $p\ge2$ map $d_{\text{key}}$ to a much higher  $d_{\text{dot}} = O(d_\text{key}^p)$ \citep{zoology, polysketch}.  \citet{linear-xmr-fastweight} propose the Deterministic Parameter-Free Projection (DPFP), while \citet{recurrent_linear_xfmr} use parameterized outer product to expand  $d_{\text{dot}}$ in a parameter-efficient/free manner. 
 
 For better memory utilization, \citet{linear-xmr-fastweight} use the delta rule to edit the memory dynamically. However, this is shown to underperform the gating mechanism \cite{mao-2022-fine}, which is a classic method to erase irrelevant historical information in gated RNNs. Recently, \citet{orthogonal_memory} enforce orthogonality of memory vectors to potentially increase utiliziation.
 %

 \paragraph{Linear attention with decay or gates.} \citet{peng2021random} use position-wise scalar gates for incorporating recency bias into linear attention, and has been revisited in recent work \cite{mamba2, beck2024xlstm, Sun2024YouOC},
 while \citet{mao-2022-fine, recurrent_linear_xfmr} use matrix-valued gates (obtained by the outer product) for more fine-grained memory control. 
 
 %

Scalar decays can be easily incorporated into chunkwise linear attention for training efficiency \citep{sun2023retentive, lightning2}. With matrix-valued gates, the training efficiency becomes much more challenging. 
 Both \citet{mao-2022-fine} and \citet{gatedloop}'s training algorithms involve materializing hidden states of all steps in HBM, which  suffers from high I/O costs. Moreover, both approaches cannot take advantage  of tensor cores. Our hardware-efficient training algorithm reduces or eliminates materialization and enables usage of tensor cores.


\paragraph{I/O-aware chunkwise linear attention.} 

The chunkwise form of  linear attention is well-known in the literature.  \citet{GAU} first propose the chunkwise linear attention form, arguing that the training algorithm of \citet{katharopoulos2020transformers} is slow in practice. 
\citet{sun2023retentive} and \citet{lightning2} generalize this form to linear attention with exponential decay (or ALiBi).  \citet{polysketch,VQ-Transformer} also derive similar chunkwise forms.

 However, most chunkwise linear attention is not I/O-aware. To the best of our knowledge, only \textsc{LightningAttention2} \cite{lightning2} (concurrent to our work) is I/O aware, and it is very similar to the non-materialization version of our \textsc{FlashLinearAttention}.  We additionally propose a materialization version, which leverages sequence-level parallelism and thus allows for higher training throughput at the cost of a slightly increasing memory footprint.  


\paragraph{Other subquadratic models.} Besides the Linear attention Transformer \cite{katharopoulos2020transformers, linear-xmr-fastweight} discussed in this work, previous studies have explored sparsifying attention with either a predefined fixed pattern \cite{child2019generating, beltagy2020longformer, zaheer2020big} or a context-aware learnable pattern \cite{roy2020efficient, kitaev2020reformer, ren2023sparse} for sequence modeling with subquadratic complexity in the sequence length dimension. Leveraging convolutions for efficient sequence modeling has also been studied in works such as Dynamic Convolution \cite{wu2019pay}, Long Convolution \cite{fu2023simple, qin2023toeplitz, hyena, massaroli2023laughing, li2023what, romero2021ckconv}, and State Space Models \cite{gu2021efficiently, gupta2022diagonal, gu2021combining, hasani2022liquid, s5, ma2023mega}.


\subsection{Sequence parallelism}

The chunk-wise parallel form of linear Transformers resembles the two-stage parallel prefix sum (or parallel scan) algorithm \citep{Blelloch1990PrefixSA}, which also combine chunk-wise parallel computations with inter-chunk communication \citep{Chaurasia2015CompilingHP}.  It also resembles sequence parallelism used for accelerating attention-based Transformers  \citep{li-etal-2023-sequence}, which has recently received  much attention  for long-sequence modeling \citep{Liu2023RingAW, Li2023LightSeqSL, Brandon2023StripedAF}. Sequence-level parallelism also constitutes the main improvement of FlashAttention-2 \citep{flashattention2} over FlashAttention-1 \citep{flashattention1}. The main differences between these works are that (i) the chunk-level parallel form of linear Transformer needs only a single pass due to the linear complexity, while the sequence parallelism in Transformers needs $L/C$ passes (i.e., left-to-right scan of key/value blocks for each query block) due to the inherent quadratic complexity, and (ii) the order of matrix multiplications is different. We also note that chunkwise linear attention could greatly reduce the communication cost between devices in the distributed training setting compared to softmax attention, which could open the door for extremely long sequence training.
\input{algorithms/la-chunk-bwd}

\subsection{Hardware-ware algorithm} Many algorithms are fast in theory, but slow in practice, due to misalignment with hardware properties \cite{Hooker2020TheHL,Saphra2023FirstTT}. 
For example, matmuls with butterfly matrices have theoretically lower complexity by using FFT, but in practice it is slow due to extensive memory  transportation operations, motivating matrices  \cite{Dao2022MonarchES,Fu2023MonarchMA} which can better align butterfly operators to GPUs. In practice it is important to reduce HBM I/O cost using techniques such as tiling and recomputation  and leverage tensor cores as much as possible. Our \textsc{FlashLinearAttention} is similar in spirit to \textsc{FlashAttention} \cite{flashattention1,flashattention2} and \textsc{FlashConvFFT} \cite{flashconvfft}, which implement I/O-aware versions of neural network layers to enable practical wallclock speedups. Concurrent work by \citet{lightning2} also proposes an I/O-aware version of linear attention, which is  similar to the non-materialization version of  \textsc{FlashLinearAttention}. We additionally propose a materialization version, which leverages sequence-level parallelism and thus allows for higher training throughput at the cost of a slightly increasing memory footprint.
\label{sec:gla_algo}




\section{Details for Chunkwise (Gated) Linear Attention}
\paragraph{Backward pass of \textsc{FlashLinearAttention}.}  
The pseduocode for backward pass of linear attention is listed in Algorithm~\ref{algo:la-chunk-bwd}.


\paragraph{Pseudo codes of GLA.}
We first present the direct adaptions of \textsc{FlashLinearAttention} to training GLA without secondary-level chunking. 
Specifically, 
Alg.~\ref{algo:gla-chunk-scan-1-fwd} and \ref{algo:gla-chunk-scan-1-bwd} shows the forward/backward pass for the materialization version; Alg.~\ref{algo:gla-chunk-scan-2-fwd} and \ref{algo:gla-chunk-scan-2-bwd} for the non-materialization version.
%
%
%
%
We show the psuedo code of our secondary-level chunking in Pytorch style in Listing~\ref{a}.


\input{algorithms/gla_scan_1}
\input{algorithms/gla_scan_2}




\paragraph{Derivations of $\dblogalpha_t$.}

We show the derivations for the following gradient form.
\begin{align*}
    \vdlogb_t &= \vk_t \odot \vdk_t - \vq_t \odot \vdq_t, \\
   %
   \dblogalpha_t  &= \sum_{t \leq i \leq L} \vdlogb_i.
\end{align*}

By unrolling the recurrence, we have
\begin{align*}
\vo_t =  \vq_t \rmS_t  &= \sum_{i=1}^{t}(\vq_t \odot \vb_t) \left(\frac{\vk_i}{\vb_i}\right)^{\top} \vv_i \\
&=  \sum_{i=1}^{t}(\vq_t \odot \exp(\log \vb_t)) \left(\vk_i \odot {\exp(- \log \vb_i)}\right)^{\top} \vv_i
\end{align*}
where at the second step, we apply a trivial identity: $\exp(\log x) = x$.
%
We first derive the gradients wrt. query/key vectors,
\begin{align*}
& \vdq_t = \sum_{ i = 1}^{t} \langle \vdo_t, \vv_i\rangle  \vb_t \odot \vk_i / \vb_i,  \\
& \vdk_i = \sum_{t = i}^{L} \langle \vdo_t, \vv_i\rangle  \vq_t \odot  \vb_t  / \vb_i.
\end{align*}
Then for the gradients wrt. the logits of the accumulative gates,
%
\begin{align*}
& \vdlogb_t  = \vq_t \odot \underbrace{\sum_{i=1}^{t} \langle \vdo_t, \vv_i\rangle  \odot  \vb_t  \odot  \vk_i / \vb_i}_{  \vdq_t} - \vk_t \odot \underbrace{\sum_{i = t}^{L} \langle \vdo_i, \vv_t\rangle  \vq_i \odot  \vb_i  / \vb_t}_{\vdk_t}.
\end{align*}
where we change the index notation for the $\vdk$ term.
It now becomes clear that 
%
\begin{align*}
& \vdlogb_t =  \vq_t \odot \vdq_t  - \vk_t \odot \vdk_t.
\end{align*}
Since $\vlogb_t = \sum_{i=1}^t \vlogalpha_i$, we get $\dblogalpha_t  = \sum_{t = i}^L \vdlogb_i$.




==> sections/supp_method.tex <==
\section{General Gated Linear Attention}
\label{sec:ggla}

In the main paper, we use a simplified parameterization where $\bbeta$ is fixed to $\mathbf{1}$ in the following gated linear attention.
%
\begin{align*}
\rmS_t = (\balpha_t^{\top} \bbeta_t) \odot \rmS_{t-1} + \vk_t^{\top} \vv_t,
\end{align*}
%
Though empirically we found that making $\bbeta$ learnable does not lead to performance gain, we show here that the general form still enjoys parallel form and chunk-wise form, which could be potentially useful for future development of linear attention models.

\subsection{Parallel form}

By unrolling the recurrence we have,
%
\begin{align}
\vo_t = \vq_t \rmS_t 
= \vq_t \sum_{i=1}^{t} \big((\prod_{i+1}^{t} \rmG_{i}) \odot (\vk_i^{\intercal}\vv_i)\big) 
\end{align}
%
%
%
%
%
%
%
%
%

By taking advantage of the mixed product property of Kronercker/outer product, we have
%
\begin{align}
(\prod_{j=i+1}^{t} \rmG_j) \odot (\vk_i^{\intercal} \vv_i) &= \big((\frac{\vb_t}{\vb_i})^{\intercal}(\frac{\vd_t}{\vd_i})\big) \odot (\vk_i^{\intercal} \vv_i) \\
&=\left( \frac{\vb_t}{\vb_i}\odot \vk_i \right)^{\intercal} \left( \frac{\vd_t}{\vd_i} \odot \vv_i \right) 
\end{align}
%
where $\vb_t = \prod_{j=1}^t \balpha_j, \vd_t = \prod_{j=1}^t \bbeta_j$.
By plugging it into the expanded recurrence, we have the following form. 
%
\begin{align}
\vo_t = \vq_t \rmS_t 
&= 
\vq_t \sum_{i=1}^{t} \big((\prod_{i+1}^{t} \rmG_{i}) \odot (\vk_i^{\intercal}\vv_i)\big) \\
    &= \vq_t \sum_{i=1}^{t} \left( \frac{\vb_t}{\vb_i}\odot \vk_i \right)^{\intercal} \left( \frac{\vd_t}{\rmB_i} \odot \vv_i \right) \\ 
    &= \sum_{i=1}^{t} \left(\vq_t \left( \frac{\vb_t}{\vb_i}\odot \vk_i \right)^{\intercal}\right) \left( \frac{\vd_t}{\vd_i} \odot \vv_i \right) \label{eq:gla_parallel_1} \\
    &= \sum_{i=1}^{t} \underbrace{\left\langle \vq_t, \frac{\vb_t}{\vb_i} \odot \vk_t \right\rangle}_{\R^{1\times 1}} \underbrace{\left( \frac{\vd_t}{\vd_i} \odot \vv_t \right)}_{\mathbb{R}^{1\times d_v}}  \\    
    &= \sum_{i=1}^{t} \left(\left\langle \vq_t \odot \vb_t, \frac{\vk_i}{\vb_i}\right\rangle \frac{\vv_i}{\vd_i} \right) \odot \vd_t \qquad  \label{eq:gla_parallel_2} \\
    &= \sum_{i=1}^{t} \left( \left(\vq_t \odot \vb_t\right)\left(\frac{\vk_i}{\vb_i}\right)^{\intercal} \left(
    \frac{\vv_i}{\vd_i} \right) \right) \odot \vd_t \quad \in \mathbb{R}^{1\times d_v} 
\end{align}
%
Eq.~\ref{eq:gla_parallel_1} is by linearity and associative property of matrix multiplication, Eq.~\ref{eq:gla_parallel_2} is derived based on $\langle \va, \vb \odot \vc \rangle = \langle \va \odot \vb, \vc \rangle$. The final form has following equivalent parallel form similar to the parallel form of linear/softmax attention.
%
\begin{align}
    \tilde \rmQ &= \rmQ \odot \rmB \qquad \tilde \rmK = \rmK / \rmB \qquad \tilde \rmV = \rmV / \rmD \\
    \tilde \rmO &= (\tilde \rmQ \tilde \rmK^\intercal \odot \rmM) \tilde \rmV \qquad \rmO = \tilde \rmO \odot \rmD
    \label{eq:gla_QKV}
\end{align}
%
where $\rmQ, \rmK, \rmB \in \R^{L \times d_k}$,
%
 $\rmV, \rmD \in \R^{L \times d_v}$,
 %
 $\rmM \in \R^{L \times L}$ denotes the causal mask.


%

%
%
%
%
%
%
%
%
%
%
%
%


\subsection{Chunkwise parallel form}

Now we show that the chunkwise parallel form for efficient training of general linear attention. Suppose $\rmX$ is now split into $\frac{L}{C}$ chunks, each of length $C$. Let $\rmS_{[i]} \in \R^{d_k \times d_v}$ be the chunk-level hidden state after processing $i$ chunks, i.e., $\rmS_{[i]}:=\rmS_{iC}$. Further let $\rmK_{[i+1]}:=\rmK_{iC+1:(i+1)C} \in \mathbb{R}^{C\times d_k}$, $\rmV_{[i+1]}:=\rmV_{iC+1:(i+1)C} \in \mathbb{R}^{C\times d_v}$. The inter-chunk recurrence is then given by,
\begin{align*}
\rmS_{[i+1]} 
&= \left(\Big(\frac{\rmB_{(i+1)C}}{\rmB_{iC}}\Big)^{\intercal}\Big(\frac{\rmD_{(i+1)C}}{\rmD_{iC}}\Big) \right) \odot \rmS_{[i]} +  \big(\rmB^{\prime}_{[i+1]} \odot \rmK_{[i+1]}\big)^{\intercal} \big(\rmD^{\prime}_{[i+1]} \odot \rmV_{[i+1]}\big),
\label{eq:gla_inter_chunk_recur}
\end{align*}
 where $(\rmB^{\prime}_{[i+1]})_j = \frac{\rmB_{(i+1)C}}{\rmB_{iC+j}} \in \mathbb{R}^{1\times d_k}$ and $(\rmD^{\prime}_{[i+1]})_j = \frac{\rmD_{(i+1)C}}{\rmD_{iC+j}} \in \mathbb{R}^{1\times d_v}$ for $j\in [1, C]$, $i \in [0, L/C-1]$. (Therefore we have $\rmB^{\prime}_{[i+1]} \in \R^{C \times d_k}, \rmD^{\prime}_{[i+1]} \in \R^{C \times d_v}$.) The intra-chunk parallel computation is then given by,
 %
\begin{align}
\tilde \rmO_{[i+1]} &= \underbrace{\left((\rmQ_{[i+1]} \odot \rmB^{\dagger}_{[i+1]}) \rmS_{[i]} \right) \odot \rmD^{\dagger}_{[i+1]}}_{\text{inter-chunk}} + \underbrace{
(\tilde\rmQ_{[i+1]} \tilde\rmK_{[i+1]}^{\intercal} \odot \rmM)\tilde\rmV_{[i+1]}
}_{\text{intra-chunk}}, \\ &\rmO_{[i+1]}  = \tilde \rmO_{[i+1]} / \rmD^{\dagger}_{[i+1]},
\label{eq:gla_inter_intra} 
\end{align}
%
 where $(\rmB_{[i+1]}^{\dagger})_j = \frac{\rmB_{iC+j}}{\rmB_{iC}} \in \mathbb{R}^{1\times d_k}$ and $(\rmD_{[i+1]}^{\dagger})_j = \frac{\rmD_{iC+j}}{\rmD_{iC}} \in \mathbb{R}^{1\times d_v}$  for $j\in [1, C]$, $i \in [0, L/C-1]$. 
 %
 Subsequently, we have $\tilde\rmQ_{[i+1]}=\rmQ_{[i+1]} \odot \rmB_{[i+1]}^{\dagger}, \tilde\rmK_{[i+1]}=\frac{\rmK_{[i+1]}}{\rmB_{[i+1]}^{\dagger}}, \tilde\rmV_{[i+1]}=\rmV_{[i+1]} \odot \rmD_{[i+1]}^{\dagger} $. For initial values, we set $\rmS_0 = \vzero$, $\rmB_0=\mathbf{1}$, $\rmD_0=\mathbf{1}$. Intuitively, $\rmB^{\prime}_{[i]} $ encodes the cumulative decay from the start of a chunk which will be used to propagate the hidden states from the previous chunk $\rmS_{[i]}$;   $\rmB^{\dagger}_{[i]}$ encodes the decay to the end of a chunk which will be used to accumulate information to be added to the next hidden state $\rmS_{[i+1]}$.


The chunkwise form given here is a generalization of several existing forms for linear attention. If we set $\rmA_{ij}=1$, $\rmB_{ij} = 1$, it reduces to the chunk-wise form presented in the main paper for vanilla linear attention; if we set $\rmA_{ij}=1$, $\rmB_{ij} = \gamma^{i+1}$, it becomes RetNet's chunk-wise form \citep{sun2023retentive}. As such, our formulation can be regarded as a generalized chunk-wise parallel form for linear attention that enables fine-grained data-dependent decay. 
\paragraph{Memory-efficient computation of $\dbalpha$ and $\dbbeta$}

In the general form, we show that the gradient wrt. $\balpha$  and $\bbeta$ admits the following closed form, which allows computing $\dbalpha$ and $\dbbeta$ without instantiating $\rmS$ in HBM.
%
\begin{align*}
    \vdlogb_t &= \vk_t \odot \vdk_t - \vq_t \odot \vdq_t, \\
   %
   \dblogalpha_t  &= \sum_{t \leq i \leq L} \vdlogb_i \\
   \vdlogd_t &= \vo_t \odot \vdo_t - \vv_t \odot \vdv_t, \\
   %
   \dblogbeta_t  &= \sum_{t \leq i \leq L} \vdlogd_i.
\end{align*}
%
where  $\vlogb_t = \sum_{i=1}^t \log \balpha_i$, $\vlogd_t = \sum_{i=1}^t \bbeta_i$ (or alternatively $\vb_t = \prod_{i=1}^t \balpha_i$, $\vd_t = \prod_{i=1}^t \bbeta_i$).  We apply the trick to compute $\vdlogb_t$ and $\vdlogd_t$ for the following cumulative-sum form.

\begin{align*}
    \vo_t = \sum_{i=1}^{t} \left( \left(\vq_t \odot \vb_t\right)\left(\frac{\vk_i}{\vb_i}\right)^{\intercal} \left(
    \frac{\vv_i}{\vd_i} \right) \right) \odot \vd_t \quad \in \mathbb{R}^{1\times d_v}.
\end{align*}
%
The gradient of $\vlogb_t$ comes from two sources: one associated with $\vq_t$, the other associated with $\vk_i$. Similarly, $\vlogd_t$ comes from both $\vo_t$ and $\vv_i$.
%
\begin{align*}
\vdlogb_t  &= \vq_t \odot \underbrace{\sum_{i=1}^{t} \langle \vdo_t, \frac{\vd_t}{\vd_i} \vv_i \rangle  \odot  \vb_t  \odot  \vk_i / \vb_i}_{  \vdq_t} - \vk_t \odot \underbrace{\sum_{i = t}^{L} \langle \vdo_i, \frac{\vd_i}{\vd_t} \vv_t \rangle  \vq_i \odot  \vb_i  / \vb_t}_{\vdk_t} \\
\vdlogd_t  &= \vdo_t \odot \underbrace{\sum_{i=1}^{t} \left( \left(\vq_t \odot \vb_t\right)\left(\frac{\vk_i}{\vb_i}\right)^{\intercal} \left(
    \frac{\vv_i}{\vd_i} \right) \right) \odot \vd_t}_{\vo_t} - \vv_t \odot \underbrace{\sum_{i=t}^{L} \left( \left(\vq_i \odot \vb_i\right)\left(\frac{\vk_t}{\vb_t}\right)^{\intercal} \left(
    \frac{1}{\vd_t} \right) \right) \odot \vd_i}_{\vdv_t} 
\end{align*}
%
The trick applied there is that $\frac{\partial f(\va \odot \vb )}{\partial \vlogb} = \va \odot \frac{\partial f(\va \odot \vb )}{\partial \va}$ and  $\frac{\partial f(\va / \vb )}{\partial \vlogb}  = - \frac{\partial f(\va / \vb )}{\partial \va} \odot \va $.

 

%
%
%
%
%
%

%
%
%
%

%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%


%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%


%


%
%
%
%
%
%

%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%


%
%
%

%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%





%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


%
%
%
%
%
%
%


%





==> sections/supp_mqar.tex <==
\vspace{-2mm}
\section{Additional Experimental Results}
\label{app:d}

The complete results on all 11 tasks, including the 5-shot results for the 1.3B models, are shown in 





%



==> tables/ablation.tex <==
\begin{table}

\centering
\small 
        \begin{tabular}{ll}
        \toprule[0.5mm]
     Model variants  &   Training ppl. \\
      \bottomrule
        {GLA Transformer} (4 heads)  & 14.77 \\
\hspace{2mm} {No gate} (i.e., Linear Attention) & 23.21\\
\hspace{2mm} {\emph{Data independent} scalar decay} (i.e., RetNet) & 16.55 \\
\hspace{2mm} {\emph{Data dependent} scalar gate} & 15.56 \\
\hspace{2mm} {Small head dimension (8 heads)} & 15.29 \\
\hspace{2mm} {Large head dimension (1 head)} &  14.61 \\
        \bottomrule
        \end{tabular}
    \vspace{-2mm}
    \caption{Ablation study results on the 340M model trained for 7B tokens. We evaluate the model variants via the average perplexity of the last 200 training steps. 
    }
        \label{tab:ablation}

    %
%
\end{table}


